Bridging Swift Error Handling Model to C++

Error handling is the process of responding to and recovering from error conditions in the program. In Swift, errors are represented by values of types that conform to the Error protocol. Throwing an error lets you indicate that something unexpected happened, and the normal flow of execution can't continue. A throw statement is used to throw an error. Optional returns are used to represent the absence of a value, but when an operation fails, it's often useful to understand what caused the failure so that code can respond accordingly. Therefore, I propose to bridge the Swift Error Handling modeling to C++ to improve the interoperability between the programming languages. The main idea is to be able to throw a C++ exception that stores a thrown Swift Error that has to be represented by a C++ class. In addition to that, to support C++ programs that don't use exceptions, I propose an additional interoperability mode for throwing functions. When C++ exceptions are disabled, C++ functions should return a result value that contains either the value returned by the function or the Swift Error value: the Swift::Exception<T> class.

==> src/Schedule.tex <==
\centering
\begin{center}
\begin{table}[!h]
\centering
\begin{tabular}{|l|l|}
\hline
Week &  Task\\ \hline
%
23/08 - 12/09 & Generate Swift Error Class in C++ to throw instead \\ & the Naive Exception. \\ \hline

12/09 - 26/09 & Define and write the project proposal. \\ \hline

26/09 - 10/09 & Create support for dynamically cast Swift Error types. \\ \hline

10/09 - 17/09 & Create support for throwing a case of a Swift Error\\ & and catch it in C++. \\ \hline

17/09 - 24/10 & Prepare and record the partial presentation (video pitch). \\ \hline

24/10 - 09/11 & Read and study the \textit{std::expected} proposal. \\ \hline

09/11 - 21/11 & Create the existential Swift Error Type to be returned\\ \hline

21/11 - 05/12 & Create a naive implementation of \textit{std::expected} \\ \hline

05/12 - 09/12 & Prepare and record the final presentation (video pitch). \\ \hline

09/12 - 19/12 &  Write documentation for the code and the final report of \\ & the project \\ \hline


\end{tabular}
\end{table}
\end{center}


==> src/appendice.tex <==
We have known some people that have worn the ring in the past. They are described in Table \ref{tab:ring_and_age}

\begin{table}[hb]
\centering
\begin{tabular}{cc}
\hline
Name    & Age       \\ \hline
Frodo   & 51        \\
Boromir & 41        \\
Smeagol & $\sim$600 \\ \hline
\end{tabular}
\caption{The age (in years) of people that have worn the ring}
\label{tab:ring_and_age}
\end{table}
